Co-design of Safe and Efficient Networked Control Systems in Factory Automation with State-dependent Wireless Fading Channels

In factory automation, heterogeneous manufacturing processes need to be coordinated over wireless networks to achieve safety and efficiency. These wireless networks, however, are inherently unreliable due to shadow fading induced by the physical motion of the machinery. To assure both safety and efficiency, this paper proposes a state-dependent channel model that captures the interaction between the physical and communication systems. By adopting this channel model, sufficient conditions on the maximum allowable transmission interval are then derived to ensure stochastic safety for a nonlinear physical system controlled over a state-dependent wireless fading channel. Under these sufficient conditions, the safety and efficiency co-design problem is formulated as a constrained cooperative game, whose equilibria represent optimal control and transmission power policies that minimize a discounted joint-cost in an infinite horizon. This paper shows that the equilibria of the constrained game are solutions to a non-convex generalized geometric program, which are approximated by solving two convex programs. The optimality gap is quantified as a function of the size of the approximation region in convex programs, and asymptotically converges to zero by adopting a branch-bound algorithm. Simulation results of a networked robotic arm and a forklift truck are presented to verify the proposed co-design method.

==> problem_formulation_revision__Jing_Chen_s_conflicted_copy_2017-08-01_.tex <==
\section{System Model: A Heterogeneous System Framework}
\label{section: SHS}
\added{Fig. \ref{fig: hsf} shows a heterogeneous system framework with two subsystems.  One is a networked control system ($\mathcal{G}$) that characterizes a nonlinear physical system being controlled over a wireless network. The other one is a Markov Decision Process (MDP) ($\mathcal{M}$) that models stochastic high level dynamics of a moving object in industrial systems. }
	
\added{The cyber-physical coupling within this heterogeneous framework is due to the fact that the physical states~(e.g., locations) of the moving object modeled by MDP's states may lead to \emph{shadow fading} on the wireless channel that is used by the networked control system. Such a coupling has been shown to be critical for performance guarantee in a variety of realistic situations in industrial applications, to name a few, such as robotic arms and forklift trucks, heavy facilities mills and cranes \cite{agrawal2014long}, sensor network with moving robots \cite{quevedo2013state,leong2016network} and indoor wireless networks with moving human bodies \cite{kashiwagi2010time}. Under such industrial settings, the radio channel characteristics are non-stationary and may experience abrupt changes due to the motion of the moving object. Such \emph{state-dependent} property of these wireless communications in industrial systems clearly invalidates the use of traditional co-design frameworks, such as \cite{molin2009lqg,gatsis2014optimal, zhang2006communication}, that rely on the assumption that the channel states are decoupled from the physical states. The heterogeneous system framework depicted in Fig. \ref{fig: hsf} is thus motivated by the co-design challenge under state-dependent fading channels.}

\deleted{Figure \ref{fig: hsf} shows a heterogeneous system framework with two subsystems. One is a networked control system ($\mathcal{G}$) that characterizes a physical robotic manipulator being controlled over a wireless network. The other one is a Markov Decision Process (MDP) ($\mathcal{M}$) that models the high transitions of a forklift truck. The MDP's states may lead to \emph{shadow fading} on the wireless channel that is used by the networked control system. This cyber-physical coupling is modeled by a state dependent channel model in Section \ref{sub: channel-model}.}
%Note that the  MDP's states may lead to \emph{shadow fading} on the wireless channel that is used by the networked control system. Under this framework, the main objective of this paper is to assure both safety and efficiency for the networked control system $\mathcal{G}$ and MDP $\mathcal{M}$.
\begin{figure}[!t]
	\centering
	\includegraphics[scale=.25]{figure/heterogeneous-systems.png}
	%\caption{Networked Control System (Robotic Manipulator) and Markov Decision Process (Forklift Trucks)}
	\caption{Heterogeneous System Framework: Networked Control System and Markov Decision Process}
	\label{fig: hsf}
\end{figure}
 \subsection{The $\mathcal{G}$ System Model}
The dynamics of the ${\mathcal G}$ system are modeled as follows,
\begin{align*}
\mathcal{G}:=\begin{cases} \dot{x}_{p}&=f_{p}(t, x_p, \hat{u}, w) \\
                                              y&=g_{p}(t, x_p)    , \quad \text{Physical Plant} \\
                                              \dot{x}_{c}&=f_{c}(t, x_{c}, \hat{y}) \\
                                              u&=g_{c}(t, x_{c}),  \quad \text{Remote Controller}. \\
\end{cases}
\end{align*}
where $x_{p} \in \mathbb{R}^{n_{x}}$ and $y \in \mathbb{R}^{n_{y}}$ are the physical states and measurements, respectively. $x_{c} \in \mathbb{R}^{n_{c}}$ and $u \in \mathbb{R}^{n_{u}}$ are the internal state and output for the remote controller, respectively. $w \in \mathbb{R}^{n_w}$ is the external disturbance that is assumed to be essentially ultimately bounded, i.e., $\exists M_w > 0$, $|w|_{\mathcal{L}_{\infty}} \leq M_w$. $f_{p}(\cdot, \cdot, \cdot, \cdot):\mathbb{R}_{\geq 0}\times \mathbb{R}^{n_{x}} \times \mathbb{R}^{n_{u}} \times \mathbb{R}^{n_w} \rightarrow \mathbb{R}^{n_x}$, $g_{p}(\cdot, \cdot): \mathbb{R}_{\geq 0} \times \mathbb{R}^{n_x} \rightarrow \mathbb{R}^{n_y}$, $f_{c}(\cdot, \cdot, \cdot):\mathbb{R}_{\geq 0}\times \mathbb{R}^{n_c} \times \mathbb{R}^{n_{u}} \rightarrow \mathbb{R}^{n_c}$ and $g_{c}(\cdot, \cdot): \mathbb{R}_{\geq 0} \times \mathbb{R}^{n_x} \rightarrow \mathbb{R}^{n_u}$ are Lipschitz functions for the physical plant and remote controller respectively.  Without loss of generality, we assume the origin is the unique equilibrium for system $\mathcal{G}$, i.e. $f_{p}(0, 0, 0, 0)=0^{n_x}, f_{c}(0, 0, 0)=0^{n_{c}}, g_{p}(0, 0)=0^{n_y}, g_{c}(0, 0)=0^{n_u}$.

Let $\{t_k\}$ denote an increasing sequence of
time instants where $t_k < t_{k+1}$ for all $k \in \mathbb{Z}_{\geq 0}$.  Let $\Omega_{p}=\{p_{i}\}_{i=1}^{M}$ be a transmission power set including $M$ power levels where $p_{i} \in \mathbb{R}_{\geq 0}$ is the power level. As shown in Figure \ref{fig: hsf}, the measurement $y$ and controller output $u$ are sampled and transmitted over an unreliable
communication channel with a selected power level $p_k \in \Omega_{p}$ at time instant $t_k$. The wireless network is subject to fading and randomly drops the sampled information at each time instant. Let $\{\gamma(k)\}$ denote a binary random process taking value from $\{0, 1\}$.  The value of the process $\gamma(k)$ at the $k$th consecutive sampling instant indicates whether or not a packet dropout has occurred. In particular,
\begin{align*}
\gamma(k)=\begin{cases} 1 & ,\quad \text{packet successfully decoded without error} \\
0 & , \quad \text{packet is dropped}. \\
\end{cases}
\end{align*}
Let $\hat{y}(t_{k})$ and $\hat{u}(t_{k})$ denote the estimates of the corresponding variables at time instant $t_{k}$. Note that we assume the time used for communication and computing control action is negligible compared to the sampling time interval and the network condition is unchanged during this small time interval. The estimation error induced by the communication during the sampling time interval $[t_{k}, t_{k+1})$ is defined as $e_{y}(t)=y(t)-\hat{y}(t_{k})$ and $e_{u}=u(t)-\hat{u}(t_{k})$. Let $e(t) = [ e_y(t); e_u(t)]^T$ denote the aggregated estimation error at time $t$. After
the information is successfully received, this aggregated estimation error will be reset to zero.  Let $t_k^+$ denote
the real time immediately after the sampling instant, $t_k$. The estimation error $e(t_k^+)$
will be reset to zero immediately after each successful transmission.  So we may formally express $e(t_k^+)$ as $e(t_{k}^{+})=(1-\gamma(k))e(t_{k})$.
Let $x:=[x_{p}; x_{c}]$ denote the aggregated state for the closed loop system $\mathcal{G}$, and then one has the following equivalent system representation in terms of $x$ and $e$,
\begin{align}
\hat{\mathcal{G}}:=\begin{cases}
\dot{x}&=f(t, x, e, w) \\
\dot{e}&=g(t,x, e, w), \forall t \in (t_{k}, t_{k+1})  \\
e(t_{k}^{+})&=(1-\gamma(k))e(t_{k}), \quad k \in \mathbb{N}^{+}.\\
\end{cases}
\label{eq: G_hat}
\end{align}
where 
\begin{align*}
f(t, x, e, w)&=\left [\begin{array}{c}   f_{p}(t, x_{p}, g_{c}(t, x_{c})-e_{u}(t), w)  \\
                                                       f_{c}(t, x_{c}, g_{p}(t, x_p)-e_{p}(t))
 \end{array} \right] \\
 g(t, x, e, w)&=\left [\begin{array}{c}      \frac{\partial g_{p}(x_p, t)}{\partial x_{p}}f_{p} (t, x_{p}, g_{c}(t, x_{c})-e_{u}(t), w) + \frac{\partial g_{p}(x_p, t)}{\partial t}                \\
                                                             \frac{\partial g_{c}(x_c, t)}{\partial x_{c}}f_{c}(t, x_{c}, g_{p}(t, x_{p})-e_{u}(t))+\frac{\partial g_{c}(x_c, t)}{\partial t}
 \end{array} \right].
\end{align*}
Note that  we further assume that the functions $g_{p}(\cdot, \cdot)$ and $g_{c}(\cdot, \cdot)$ are continuously differentiable and thus the function $g(\cdot, \cdot, \cdot, \cdot)$ in \eqref{eq: G_hat} is well defined. Since the (set)~stability of the system $\hat{\mathcal{G}}$ implies the (set)~stability of the system $\mathcal{G}$, we will only discuss the stability of the system $\hat{\mathcal{G}}$ in the remaining of this paper.  
%As of now, We say the system safety in VNS is assured under the heterogeneous system framework if appropriate notions of stability are achieved for the networked control system model defined in \ref{eq: G_hat}. 
\subsection{The $\mathcal{M}$ System Model}
The $\mathcal{M}$ system is modeled by an MDP process. An MDP is defined by a five tuple $\mathcal{M}=\{S, s_{0}, A, P, c\}$, where
\begin{itemize}
\item $S=\{s_{i}\}_{i=1}^{N}$ is the state space for the MDP.
\item $s_{0} \subset S$ is the set of initial states.
\item $A=\{a_{i}\}_{i=1}^{M_{a}}$ is the action set.
\item $P: S \times A \times S \rightarrow [0, 1]$ is the transition probability , i.e. $P(s_{i}, a, s_{j})={\rm Pr}\{s_{j}| a, s_{i}\}$.
\item $c: S \times A \rightarrow \mathbb{R}_{\geq 0}$ is the reward function. 
\end{itemize}

Unlike system $\mathcal{G}$ that models low level physical dynamics, the MDP process is used to model discrete-event decision making
processes managing high-level control objectives such as transporting products from one location to another with minimum time or energy. \added{The state space $S$ in the MDP system corresponds to a finite number of partitioned regions that the vehicle system, such as forklift trucks or cranes \cite{agrawal2014long} or robots \cite{quevedo2013state}, can operate by taking actions from an action set $A$.  The transition probability matrix $P$ is used to model the stochastic uncertainties caused by sensor or actuation noises when the actions are physically implemented. The costs in the MDP model are defined to characterize the high level control objectives for the vehicle system. For instance, if the control objective is to transport the products to a target region, then small costs will be assigned in the minimization optimization problem, to the situation when the vehicle is transitted to the target region.}
%
%Given the MDP system model, the control policy for system $\mathcal{M}$ refers to an infinite sequence $u=(u_{1}, u_{2}, \ldots)$ where $u_{k}$ is the decision made at time instant $k$. Note that the decision making may depend on the information observed along the time. Specifically, let $h_{t}^{m}=(s_{1}, a_{1}, \ldots, s_{t-1}, a_{t-1}, x_{t})$ denote a history of states and actions up to time $t$, then the decision making variable $u_{k}$ in control policy $u$ could be defined as a probability distribution over the action set $A$ given the history information, i.e., $u_{t}={\rm Pr}\{a | h_{t}\}, \forall a \in A$. Clearly, one may classify different control policies based on the type of information used to make decisions. For more details about the types of control policies in MDP, please refer to \cite{puterman2014markov}. In this chapter, we are interested in the following two types of control policies \cite{altman1999constrained},
%\begin{definition}[Markov Policies]
%If $\forall t$, the action $u_{t}$ in the control policy is only a function of current state $s_{t}$, not the entire history, then this control policy is Markovian and the class of all policies having the Markov property are called Markov policies. 
%\end{definition}
%\begin{definition}[Stationary Policies]
%If a control policy is a Markov policy and the decision $u_{t}$ is independent of time $t$, then the class of all such policies are called Stationary policies. 
%\end{definition}
%In fact, for many MDP optimization problems, it suffices to restrict our attention to Markov or Stationary policies for optimal strategies \cite{altman1999constrained}. 
%Each state~(partitioned regions) of MDP may correspond to a specific fading level induced by the presence of the vehicle system.
\subsection{State Dependent Dropout Channel Model}
\label{sub: channel-model}
As shown in Fig. \ref{fig: hsf}, the wireless channel used by the networked control system $\mathcal{G}$ is functionally dependent on the state of the MDP system. This relationship corresponds to the situation that vehicle's physical positions directly lead to \deleted{the} shadow fading, thereby generating a great deal of stochastic uncertainties in system $\mathcal{G}$. Equation (\ref{eq: G_hat}) shows that the stochastic uncertainty in system $\hat{\mathcal{G}}$ is governed by a binary random process $\{\gamma(k)\}$, which characterizes the stochastic variations in channel conditions. 

The state-dependency in the shadow fading channel is captured by a novel \emph{State-Dependent Dropout Channel} (SDDC) model that is formally defined as follows.
\begin{definition}
\label{def: SDDC}
Given a binary random process $\{\gamma(k)\}_{k=0}^{\infty}$, an MDP system $\mathcal{M}=\{S, s_{0}, A, P_{m}, c\}$ and a transmission power set $\Omega_{p}=\{p_{i}\}_{i=1}^{M}$,  the wireless channel is SDDC if 
\begin{align}
\label{eq: SDDC}
{\rm Pr}\{\gamma(k)=1 | s(k)=s, p(k)=p\} = 1-\theta(s, p), \forall s \in S, p \in \Omega_p.
\end{align}
where $\theta(s, p) \in (0, 1)$ is the outage probability \cite{tse2005fundamentals} that monotonically decreases with respect to the transmission power level $p$.
\end{definition}
\begin{remark}
	\added{
The definition of the SDDC is closely related to  the \emph{outage probability}, which is a widely used performance metric for fading channels \cite{tse2005fundamentals}. It characterizes the likelihood of the Signal-to-Noise Ratio~(SNR) \added{being} below a specified threshold $\gamma_0$, i.e. ${\rm Pr}\{\text{SNR} \leq \gamma_0\}$. The difference between the SDDC model and traditional \emph{outage probability} lies in the state-dependent feature of \eqref{eq: SDDC} where the probability is defined for each each MDP state~(partitioned region). The probability defined in \eqref{eq: SDDC} can be obtained by measuring the SNR for each MDP state, see \cite{kashiwagi2010time, agrawal2014long} and reference therein for details about the statistical methods. In practice, the transmitter can estimate the probability by either directly using the visual sensor to observe the positions of the controlled moving object, or using the estimation techniques discussed in \cite{agrawal2014long,agrawal2009correlated}. See Example \ref{example: raleigh-fading} for more details about how to construct the SDDC from the \emph{outage probability}.}
\end{remark}

\begin{remark}
	\added{
The SDDC model in \eqref{eq: SDDC} relates the channel state~(packet dropout probability) to the MDP states and transmission power levels. From a control standpoint, this correlation enables that the channel conditions can be controlled by designing different control and transmission power strategies. By using such a freedom in the channel model, this paper develops a co-design framework that coordinates control and communication strategies to achieve both safety and efficiency for the entire heterogeneous system. The co-design idea of using the state-dependent channel model distinguishes our work from other results, such as \cite{quevedo2013state, kashiwagi2010time, agrawal2014long, leong2016network} where the channel state is assumed a fixed and uncontrollable random process.}
\end{remark}

\begin{example}[SDDC model with Raleigh fading]
\label{example: raleigh-fading}
Channel fading is often the result of the superimposition of signal attenuation in both large~(shadowing) and small scale levels \cite{tse2005fundamentals}. Let $h_k$ denote the small scale fading gain induced by multi-path propagation at time instant $t_k$.  Suppose $\{h_{k}\}_{k=0}^{\infty}$ is an \emph{i.i.d} process that
satisfies a Raleigh distribution with a scale parameter $1$, i.e. $h_{k} \sim \text{Raleigh}(1), \forall k \in \mathbb{Z}_{\geq 0}$. Let $\psi(\cdot): S \rightarrow [0, 1]$ denote a shadow level function that characterizes the level of shadowing effect on the channel gain for each MDP state, i.e. $0 \leq \psi(s) \leq 1, \forall s \in S$. Thus, the state dependent channel gain is $\overline{h}_{k}(s):=\psi(s)h_{k}$, and for a given transmission power level $p$ and noise power $N_0$, the SNR is $p\overline{h}_{k}(s)^{2}/N_0$. With the assumption that the small scale fading gain is conditionally independent on shadowing state $s \in S$,  for a given SNR threshold $\gamma_0$, one has
\begin{align*}
&{\rm Pr}\{\gamma(k)=1 | s(k)=s,p(k)=p\}\\=&{\rm Pr}\{\frac{p(k)h_{k}^{2}\psi(s(k))^{2}}{N_{0}} \geq \gamma_{0} \Big| s(k)=s, p(k)=p\} \\                                                             =&\int_{\frac{\gamma_{0}N_{0}}{p}}^{\infty} \psi(s) e^{-\psi(s) x} dx = e^{-\frac{N_{0}\gamma_{0}\psi(s)}{p}}.
\end{align*}
Then, we have the explicit function form $\theta(s, p)=1-e^{-\frac{N_{0}\gamma_{0}\psi(s)}{p}}$ for SDDC model. 
\end{example}

The SDDC in \eqref{eq: SDDC} characterizes a \emph{cyber-physical coupling} between the networked control system $\mathcal{G}$ and the MDP system $\mathcal{M}$. In the presence of such coupling, the first objective of this paper is to find conditions under which system $\mathcal{G}$ achieves \replaced{\emph{stochastic safety} that is formally defined as belows.}{\emph{almost sure asymptotic stability} without external disturbance~($w=0$) and \emph{stochastic stability in probability} with essentially ultimated bounded disturbance. These stability notions are formally defined as follows.}
%{\color{red}
\begin{definition}[Stochastic Safety]
	\label{def:stochastic-safety}
	Consider the networked control system $\hat{\mathcal{G}}$ in (\ref{eq: G_hat}) and the SDDC model in (\ref{eq: SDDC}), let $\Omega_{s}=\{x \in \mathbb{R}^{n_x+n_c} \vert |x| \leq r \}$ with $r \geq 0$ denote a safe set for $\hat{\mathcal{G}}$ system, and $x_0=x(0)$ denote the initial state of the networked control system, 
	\begin{itemize}
		\item[\textbf{E1}] The $\hat{\mathcal{G}}$ system with $w \equiv 0$ is \emph{asymptotically safe in expectation} with respect to $\Omega_{s}$, if $\forall x(0) \in \Omega_{s}$, there exists a class $\mathcal{KL}$ function $\overline{\beta}(\cdot, \cdot)$ such that
		\begin{align}
		\label{eq: asymptotic-safety-in-expectation}
		\mathbb{E}\big[ |x(t)| \big] \leq \overline{\beta}(|x_0|, t), \quad \forall t \in \mathbb{R}_{\geq 0}
		\end{align}
		and thereby $\lim_{t \rightarrow +\infty}\mathbb{E}\big[ |x(t)| \big]=0$.
		\item[\textbf{E2}] The $\hat{\mathcal{G}}$ system with $|w(t)|_{\mathcal{L}_{\infty}} \leq M_w$ is \emph{asymptotically bounded in expectation} with respect to $\Omega_{s}$, if $\forall x(0) \in \Omega_{s}$, there exists a class $\mathcal{KL}$ function $\overline{\beta}(\cdot, \cdot)$ and a class $\mathcal{K}$ function $\kappa(\cdot)$ such that 
		\begin{align}
		\label{ineq: stochastic-safety-in-expectation}
		\mathbb{E}\big[ |x(t)|\big] \leq \overline{\beta}(|x_0|, t) + \kappa(M_w), \quad \forall t \in \mathbb{R}_{\geq 0}
		\end{align}
		and $\lim_{t \rightarrow +\infty}\mathbb{E}\big[ |x(t)|\big]=\kappa(M_w)$.
		\item[\textbf{P1}] The $\hat{\mathcal{G}}$ system with $w \equiv 0$ is \emph{almost surely asymptotically safe} with respect to $\Omega_{s}$, if $\forall \epsilon, \tau > 0$ and $x_{0} \in \Omega_{s}$, there exists a class $\mathcal{KLL}$ function $\beta_{\epsilon}(\cdot, \cdot, \cdot)$ such that 
		\begin{align}
		\label{ineq: almost-sure-safety}
		{\rm Pr}\big\{\sup_{t \geq \tau} |x(t)| \geq \epsilon+r \big\} \leq \beta_{\epsilon}(|x_0|, \tau, r) 
		\end{align}
		and $\lim_{\tau \rightarrow \infty} {\rm Pr}\big\{\sup_{t \geq \tau} |x(t)| \geq \epsilon+r \big\}=0$.
		\item[\textbf{P2}] The $\hat{\mathcal{G}}$ system with $|w(t)|_{\mathcal{L}_{\infty}} \leq M_w$ is \emph{stochastically safe in probability} with respect to $\Omega_{s}$, if $\forall \epsilon_1 > 0$, there exists a class $\mathcal{KL}$ function $\overline{\beta}_{\epsilon_2}(M_w, r)$ such that 
		\begin{align}
		\label{ineq: stochastic-safety-in-probability}
		\lim_{t \rightarrow \infty}{\rm Pr}\big\{ |x(t)| \geq \epsilon_1+r\big\} \leq \overline{\beta}_{\epsilon_2}(M_w, r).
		\end{align}
	\end{itemize}
	\end{definition}
%}
	
%\deleted{\textbf{Definition II.5} (Almost Sure Asymptotic Safety) Consider the networked control system $\hat{\mathcal{G}}$ in (\ref{eq: G_hat}) with $w=0$ and the SDDC model in (\ref{eq: SDDC}), let $\Omega_{s}=\{x \in \mathbb{R}^{m} \vert |x| \leq r \}$ with $r \geq 0$ denote a safe set for $\hat{\mathcal{G}}$ system, the $\hat{\mathcal{G}}$ system is \emph{almost surely asymptotically safe} with respect to $\Omega_{s}$ if $\forall x \in \Omega_{s}$}
% \begin{equation}
%	\label{eq: almost-sure-safety}
%\deleted{{\rm Pr}\{x(t) \in \Omega_{s} \} \rightarrow 1, \, \text{as} \; t \rightarrow +\infty.}
%	\end{equation}
%\deleted{or} 
% \begin{equation}
%  \label{eq: stochastic-safety}
%  {\rm Pr}\{x(t) \notin \Omega_{s} \} \rightarrow 0, \, \text{as} \; t \rightarrow +\infty.
%  \end{equation}

%\begin{definition}[Stochastic Safety in Probability]
%Consider the $\hat{\mathcal{G}}$ system in (\ref{eq: G_hat}) with external disturbance $w \neq 0$ and the SDDC model in (\ref{eq: SDDC}), for a given bounded set $\Omega_{s}$, the system is \emph{stochastically safe in probability} with respect to $\Omega_{s}$ if $\forall \epsilon > 0$, there exists $\delta > 0$ such that $\forall x(0) \in \Omega_{s}$,
%$
%	{\rm Pr}\{x(t) \notin  \Omega_{s}+\delta\mathbb{B} \} \leq \epsilon , \, \text{as} \; t \rightarrow +\infty.
%$ where $\mathbb{B}=\{y \in \mathbb{R}^{n_p+n_c} \vert \|y\|_{2} \leq 1\}$ is a closed unit ball.
%\end{definition}
%{\color{red}
\begin{remark}
The safety notions \textbf{E1} and \textbf{E2} are concerned with system behavior on average~(in the first moment) while the safety notions \textbf{P1} and \textbf{P2} focus on the specification on the sample path of the system. Note that these two types of safety definitions specify both the system's transient and steady behavior. In particular, for systems without external disturbance, the safety definition \textbf{E1} requires that the first moment of the norm of the system trajectories must asymptotically converge to the origin if the initial states start within the safety set while the \emph{almost sure safety} definition \textbf{P1} is a stronger safety notion than the definition \textbf{E1} in the sense that it requires almost all sample paths starting from the safety set $\Omega_{s}$ stay in the safe region with probability one. For systems with \replaced{non-vanishing}{non-varnishing} but ultimately bounded disturbance, the definitions \textbf{E2} and \textbf{P2} provide relaxed notions of safety in the first moment and in probability. The definition \textbf{E2} requires that the first moment of the system trajectories is asymptotically bounded with its bound depending on the magnitude of external disturbance. The safety notion \textbf{P2} basically means that the probability of sample paths of the system leaving the safe region is asymptotically bounded and the probability bound is a function of the size of the external disturbance and safety region. These safety notions are closely related to the concepts of stochastic stability defined in \cite{kushner1967,khasminskii2011stochastic}.
\end{remark}
%}

Under the safety conditions for system $\mathcal{G}$, the second objective of this paper is to seek optimal control and communication policies to achieve system efficiency for both system $\mathcal{G}$ and $\mathcal{M}$. A control policy for the MDP system $\mathcal{M}$ is an infinite sequence $\pi^{m}=\{u^{m}_1, u^{m}_2, \ldots\}$ where $u^{m}_k$ is the decision made at time instant $k$. The decision making $u^{m}_k$ is defined as a probability distribution over the action set $A$ given the history information, i.e.,~$u_{k}^{m}={\rm Pr}\{a \vert s_{k}, a_{k-1}, \ldots, s_0\}, \forall a \in A$. Similarly, a power policy for system $\mathcal{G}$ can be defined as $\pi^{p}=\{u^{p}_1, u^{p}_{2}, \ldots, \}$ with $u^{p}_{k}={\rm Pr}\{p \vert s_{k}, a_{k-1}, \ldots, s_0\}$. The policy is \emph{stationary} if $\pi^{m}_{\infty}=\{u_{\infty}^{m}, u_{\infty}^{m}, \ldots \}$~($\pi^{p}_{\infty}=\{u_{\infty}^{p}, u_{\infty}^{p}, \ldots \}$) with $u_{\infty}^{m}={\rm Pr}\{a \vert s\}$~($u_{\infty}^{p}={\rm Pr}\{p \vert s\}$), $\forall a \in A, s \in S$ and $p \in \Omega_p$. \added{This paper will focus on the stationary policy space.}

With the definitions of control $\pi^{m}$ and communication $\pi^{p}$ policies, the system efficiency is defined as a constrained infinite horizon optimization problem as follows,
\begin{equation}
\label{eq: opt-original}
\begin{aligned}
& \underset{\pi^{p}, \pi^{m}}{\text{min}}
& & J_{\alpha}(s_{0}, \pi^{m}, \pi^{p})=(1-\alpha)\sum_{k=0}^{\infty}\alpha^{k}\mathbb{E}\{\lambda c_{p}(p_{k})+c(s_{k}, a_{k})\}\\
& \text{s.t.} 
& & \text{Safety conditions assuring}~\eqref{eq: asymptotic-safety-in-expectation}~\text{or}~\eqref{ineq: stochastic-safety-in-expectation}~\text{or}~\eqref{ineq: almost-sure-safety}~\text{or}~\eqref{ineq: stochastic-safety-in-probability}.
\end{aligned}
\end{equation}
where $c_{p}(\cdot): \Omega_p \rightarrow \mathbb{R}_{\geq 0}$ is the power cost and $c(\cdot, \cdot)$ is the cost defined in the MDP system.  \replaced{$\alpha \in (0, 1)$ is the discounted factor that provides a weight between short term rewards and rewards that might be obtained in a more distance future. $\lambda> 0$ is a parameter used to adjust the weight between communication and control costs.}{$\lambda > 0$ and $\alpha \in (0, 1)$ are the weight and discounted factors respectively.} 

%Compared to traditional co-design problems, such as \cite{molin2009lqg,gatsis2014optimal, zhang2006communication} and the reference therein, that assume the independence between channel states and physical states in one single networked control system, the novelty of our proposed framework in \eqref{eq: opt-original} lies in the following two asepcts, 
%	\begin{itemize}
%\item The proposed framework explicitly consideres the impact of the non-stationary and state-dependent property of wireless networks on the co-design problem,  which has been shown to be critical in industrial applications\cite{agrawal2014long, quevedo2013state, kashiwagi2010time}.  The presence of such a \emph{state-dependent} property inevitably introduces the coupling between control and communication policies that leads to nontrivial non-convex constraints in our co-design problem.
%\item Rather than focusing on co-design for one single networked control system, our proposed framework is motivated by the complex industrial settings where the cyber-physical couplings exist in heterogeneous systems with different dynamic levels. The co-design framework with such heterogeneous structures favorably represents a variety of realistic situations in industrial applications, to name a few, such as manufacturing systems with heavy facilities mills and cranes discussed in \cite{agrawal2014long}, sensor network with moving robot \cite{quevedo2013state} and indoor wireless networks with moving human bodies \cite{kashiwagi2010time}.
%\end{itemize} 
